Global-to-Local or Local-to-Global? Enhancing Image Retrieval with Efficient Local Search and Effective Global Re-ranking

The dominant paradigm in image retrieval systems today is to search large databases using global image features, and re-rank those initial results with local image feature matching techniques. This design, dubbed global-to-local, stems from the computational cost of local matching approaches, which can only be afforded for a small number of retrieved images. However, emerging efficient local feature search approaches have opened up new possibilities, in particular enabling detailed retrieval at large scale, to find partial matches which are often missed by global feature search. In parallel, global feature-based re-ranking has shown promising results with high computational efficiency. In this work, we leverage these building blocks to introduce a local-to-global retrieval paradigm, where efficient local feature search meets effective global feature re-ranking. Critically, we propose a re-ranking method where global features are computed on-the-fly, based on the local feature retrieval similarities. Such re-ranking-only global features leverage multidimensional scaling techniques to create embeddings which respect the local similarities obtained during search, enabling a significant re-ranking boost. Experimentally, we demonstrate solid retrieval performance, setting new state-of-the-art results on the Revisited Oxford and Paris datasets.

==> preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sections/S_rank_more_candidates.tex <==
\section{Re-ranking Different Number of Candidates in MDS}
\label{sec:rerank_supp}

This section serves as an extension to Section \textcolor{red}{4.2} and evaluates using MDS with different number of candidates on $\mathcal{R}$evisited Oxford 5k and $\mathcal{R}$Paris 6k \cite{radenovic2018revisiting}. 
As presented in Table \ref{tab:rank_more_candidates_new_supp}, MDS achieves similar performance when only re-ranking 600 images. It significantly outperforms RN101-CVNet re-ranking (top 400) by $7.6\%$ on $\mathcal{R}$Oxford Hard, and surpasses SuperGlobal (re-rank top 400) by $3.3\%$ in the same dataset. 


\input{sections/S_tab_rank_more_candidates}

==> sections/S_tab_rank_more_candidates.tex <==
\begin{table}[hp]
\footnotesize
\addtolength{\tabcolsep}{-0.15em}
\centering
{%\scriptsize
\begin{tabular}{l c c c c c}
%\toprule
\multirow{2}{*}{\small Top $K$} &    \multicolumn{2}{c}{ \small Medium} & & \multicolumn{2}{c}{ \small Hard} \\[+0.3em] \cmidrule[0.5pt]{2-3} \cmidrule[0.5pt]{5-6}
 & \multicolumn{1}{c}{\large \vphantom{M} \scriptsize $\mathcal{R}$Oxf } & \multicolumn{1}{c}{\scriptsize $\mathcal{R}$Par} && \multicolumn{1}{c}{\scriptsize $\mathcal{R}$Oxf} & \multicolumn{1}{c}{\scriptsize $\mathcal{R}$Par}  \\
\midrule
\num{400}  & \num{92.3} & \num{93.3}  && \num{82.9}  & \num{86.7}  \\
\num{600}  & \num{92.7} & \num{96.0}  && \num{83.5}  & \num{90.1}  \\
\num{1600}  & \num{92.9} & \num{97.1}  && \num{83.0}  & \num{91.7}  \\
\hline
\end{tabular}

}


% \vspace{-5pt}
\caption{Results (\% mAP) when using different $K$ values during re-ranking on the $\mathcal{R}$Oxford and $\mathcal{R}$Paris datasets \cite{radenovic2018revisiting} using our L2G method, with both Medium and Hard evaluation protocols. }
\label{tab:rank_more_candidates_new_supp}
\end{table}

==> sections/S_tab_twice_reranking.tex <==
\begin{table}
\footnotesize
\addtolength{\tabcolsep}{-0.15em}
\centering
{%\scriptsize
\scalebox{0.9}{
\begin{tabular}{l c c c c c}
%\toprule
\multirow{2}{*}{\small Method} &    \multicolumn{2}{c}{ \small Medium} & & \multicolumn{2}{c}{ \small Hard} \\[+0.3em] \cmidrule[0.5pt]{2-3} \cmidrule[0.5pt]{5-6}
 & \multicolumn{1}{c}{\large \vphantom{M} \scriptsize $\mathcal{R}$Oxf } & \multicolumn{1}{c}{\scriptsize $\mathcal{R}$Par} && \multicolumn{1}{c}{\scriptsize $\mathcal{R}$Oxf} & \multicolumn{1}{c}{\scriptsize $\mathcal{R}$Par}  \\
\midrule

%\midrule
% ResNet50-DELG \cite{cao2020unifying} &   \num{43.3} & \num{24.2}  & \num{58.0}  & \num{29.9} &&  \num{17.1} & \num{9.4} & \num{29.7} & \num{8.4} \\
% ResNet101=DELG \cite{cao2020unifying} &     \num{61.9} &  \num{42.6} & \num{69.3}  & \num{45.4} && \num{33.7} & \num{19.0} & \num{44.3} & \num{19.1} \\ 
{AMES\cite{suma2024ames} paper after SG reranking\cite{superfeatures}}  & \num{93.6} & \num{95.3}  && \num{84.8}  & \num{90.7}  \\
\hline
AMES Retrieval + Re-ranking & & & & \\
{+ re-ranking via MDS embedding}  & \num{93.94} & \num{93.67}  && \num{84.93}  & \num{88.54}  \\
{+ SG re-ranking with this embedding} & \num{\textbf{95.90}} & \num{96.98}\  && \num{\textbf{87.63}}  & \num{93.07}  \\
\hline
SG Retrieval + AMES Re-ranking & & & & \\
{+ re-ranking via MDS embedding}  & \num{93.24} & \num{95.18}  && \num{83.64}  & \num{90.68}  \\
{+ SG re-ranking with this embedding} & \num{94.62} & \num{\textbf{98.76}}  && \num{84.75}  & \num{\textbf{95.30}}  \\
\hline
\end{tabular}}



}


% \vspace{-5pt}
\caption{Results (\% mAP) of combining MDS re-ranking and SG re-ranking \cite{shao2023superglobal} using MDS embedding on the $\mathcal{R}$Oxford and $\mathcal{R}$Paris datasets \cite{radenovic2018revisiting}, with both Medium and Hard evaluation protocols. The best results are highlighted in \textbf{bold}. }
\label{tab:two_reranking_new_supp}
\end{table}

==> sections/S_twice_reranking.tex <==
\section{Combining MDS Re-ranking with SG Re-ranking}
\input{sections/S_tab_twice_reranking}

% \noindent\textbf{Can CVNet-Rerank improve our reranking results?}
Our work is proved to be significantly outperforming AMES re-ranking \cite{suma2024ames}. For completeness, we perform experiments to study the effect of combining MDS re-ranking and SuperGlobal re-ranking, when using different features for retrieval. The results are shown in Table \ref{tab:two_reranking_new_supp}. Here AMES retrieval is done by using the pairwise similarities between all images in the query and database. We note that, by adding MDS re-ranking, the results on both $\mathcal{R}$Oxford and $\mathcal{R}$Paris are already comparable to the ones in AMES paper. The performance can be further improved by adding SG re-ranking with MDS embeddings -- on $\mathcal{R}$Oxford Hard and $\mathcal{R}$Paris Hard, the best mAP metrics are $87.63$ when using AMES for retrieval and $95.30$ when using SG for retrieval, respectively. This further demonstrates the effectiveness between combining SG re-ranking and MDS re-ranking.

